Casting of the WAM as an EAM

Logic programming provides a very high-level view of programming, which comes at the cost of some execution efficiency. Improving performance of logic programs is thus one of the holy grails of Prolog system implementations and a wide range of approaches have historically been taken towards this goal. Designing computational models that both exploit the available parallelism in a given application and that try hard to reduce the explored search space has been an ongoing line of research for many years. These goals in particular have motivated the design of several computational models, one of which is the Extended Andorra Model (EAM). In this paper, we present a preliminary specification and implementation of the EAM with Implicit Control, the WAM2EAM, which supplies regular WAM instructions with an EAM-centered interpretation.

==> boxes.tex <==
\makeatletter

\def\andb{\@ifnextchar [{\@andbx}{\@andbx[]}}
\def\@andbx[#1]{\@ifnextchar [{\@andbxx[#1]}{\@andbxx[#1][]}}
\def\@andbxx[#1][#2]#3{\mathsf{AND}_{\mathsf{#1}}^{\mathsf{#2}}(#3)}

\def\chb{\@ifnextchar *{\choicebox}{\choicebox*}}
\def\choicebox*#1{\mathsf{OR}(#1)}

\def\orb{\@ifnextchar *{\@orbx}{\@orbx*}}
\def\@orbx*{\@ifnextchar [{\@orbxx*}{\@orbxx*[]}}
\def\@orbxx*[#1]#2{\mathsf{OR}^{\mathsf{#1}}(#2)}

\def\transition{\Rightarrow \\ \mbox{\hspace{4em}}}
\newenvironment{transitions}{$}{$\\}
\def\fails{\transition \textsf{FAIL}}

\makeatother

